Provably efficient, succinct, and precise explanations

We consider the problem of explaining the predictions of an arbitrary blackbox model $f$: given query access to $f$ and an instance $x$, output a small set of $x$'s features that in conjunction essentially determines $f(x)$. We design an efficient algorithm with provable guarantees on the succinctness and precision of the explanations that it returns. Prior algorithms were either efficient but lacked such guarantees, or achieved such guarantees but were inefficient. We obtain our algorithm via a connection to the problem of {\sl implicitly} learning decision trees. The implicit nature of this learning task allows for efficient algorithms even when the complexity of $f$ necessitates an intractably large surrogate decision tree. We solve the implicit learning problem by bringing together techniques from learning theory, local computation algorithms, and complexity theory. Our approach of "explaining by implicit learning" shares elements of two previously disparate methods for post-hoc explanations, global and local explanations, and we make the case that it enjoys advantages of both.

==> ProvablePerformanceGuarantees.tex <==
%!TEX root = explainability.tex


\section{Provable performance guarantees}

In this section we establish formal guarantees on the succinctness and precision of the anchors that our algorithm $\mathscr{A}$ returns.  We accomplish this by bringing together results from complexity theory and local computation algorithms; the two main ingredients in our proofs are:  
\begin{enumerate}[leftmargin=15pt]
\item A theorem of Smyth~\cite{Smy02} which we apply to relate the ``anchor complexity" of a function and its decision tree complexity.  A key enabling observation here is a close correspondence between anchors and the notion of {\sl certificates} in computational complexity.  Certificates, also known as {\sl witnesses}, are the basis of the complexity class NP. (Smyth's result resolved a conjecture of Tardos~\cite{Tar89} that was motivated by the problem of separating P from $\text{NP} \cap \text{coNP}$.) 
\item A decision tree structure theorem of Blanc, Lange, and Tan~\cite{BLT-test}, developed in the context of local computation and sublinear algorithms.  This result bounds, under distributional and feature assumptions, the distance between $\Upsilon_f^{k,\eta}$ and $f$ in terms of $k$ and~$\eta$. 
\end{enumerate} 

\label{sec:provable performance guarantees}

\subsection{Problem setup and a general conjecture}

Our goal is to show that for all functions $f : \Omega \to \bits$ and distributions $\mathcal{D}$ over $\Omega$, our anchor-finding algorithm $\mathscr{A}$ returns {\sl precise} and {\sl succinct} anchors.  In more detail, if $f$ and $\mathcal{D}$ are such that most instances $\bx \sim \mathcal{D}$ have an $\eps$-error anchor of size $k$, we would like it to be the case that for most instances $\bx\sim \mathcal{D}$, our algorithm $\mathscr{A}$ returns an $O(\eps)$-anchor of size bounded by a slow-growing function of $k$ and $1/\eps$.  This motivates the following definition:  

% Given black box access to a model $f$, we wish to prove that our algorithm finds ``good" decision trees and ``good" anchors. A ``good" anchor is precise and succinct, as in \Cref{def:anchors}. Correspondingly, a ``good" implicit decision tree is accurate, meaning it differs from $f$ on only a small fraction of possible inputs, and has small depth. However, there are functions $f$ for which it is impossible to construct a small depth and accurate decision tree. If $f$ is a random function over $d$ features, it's not hard to show that with high probability over the choice of $f$ achieving accuracy significantly better than a coin flip requires building a tree of depth $\Omega(d)$, which can be too large to be useful. To make our task feasible, we wish to compute a decision tree with depth ``close to" the optimal.

% \begin{definition}[Optimal approximate decision tree depth]
%     \label{def:optimal dt depth}
%     Let $f: \Omega \to \bits$ and $\eps>0$. The {\sl $\eps$-optimal decision tree depth}, denoted $\depth_\eps(f)$, is the minimum depth $k$ for which there exists a depth-$k$ decision tree $T$ satisfying $\Prx_{\bx \sim \mathcal{D}}[T(\bx) \neq f(\bx)] \leq \eps$.
% \end{definition}

% Given the above definition, we are able to formally state our first conjecture. We will later prove a special case of this conjecture.
% \begin{conjecture}[Implicit DT algorithm] 
%     \label{conj:implicit dt}
%     Let $f:\Omega \to \bits$ be any target function and $\eps>0$ be any desired accuracy. For an appropriately chosen perturbation distributions, $\mathscr{P}$, the algorithm in \Cref{lem:our-implicit-alg} with depth $k = \poly(\frac{1}{\eps}, \depth_\eps(f))$ learns an implicit decision tree with accuracy $O(\eps)$.
% \end{conjecture} 
% Note that $\poly(\frac{1}{\eps}, k)$ refers to some fixed but unspecified polynomial of $\frac{1}{\eps}$ and $k$. \Cref{conj:implicit dt} is useful when $\depth_\eps(f)$ is small. A depth $k$ decision tree has $\Omega(2^k)$ parameters, so it's reasonable to expect models with lots of parameters to be close to some small depth decision tree.

% We make a similar conjecture for \textsc{ComputeAnchor}. First, we need an analogous definition to \Cref{def:optimal dt depth}.

\begin{definition}[Anchor complexity]
\label{def:anchor complexity}
    Let $f: \Omega \to \bits$ be a function over a $d$-dimensional instance space $\Omega$ and $\mathcal{D}$ be a distribution over $\Omega$.  For any instance $x \in \Omega$, we define the  {\sl $\eps$-error anchor complexity $f$ at $x$}, denoted $\mathcal{A}(f,x,\eps)$, to be the size of the smallest $\eps$-error anchor for $x$.  That is, $\mathcal{A}(f,x, \eps)$ is the size of the smallest set $A\sse [d]$ for which
    \begin{align*}
        \Prx_{\by\sim \mathcal{D}}\big[f(\by) \ne f(x)\mid \by_A = x_A\big] \le \eps.
    \end{align*}
    The {\sl $\eps$-error anchor complexity of $f$}, denoted $\mathcal{A}(f, \eps)$, is defined as
    \begin{align*}
        \mathcal{A}(f, \eps) \coloneqq \Ex_{\bx \sim \mathcal{D}}[\mathcal{A}(f,\bx, \eps)].
    \end{align*}
    When $\eps = 0$, we simply write $\mathcal{A}(f,x)$ and $\mathcal{A}(f)$.
\end{definition}

Recall that our the implicit decision tree learning algorithm, on which $\mathscr{A}$ is based, is defined in terms of an ensemble of perturbation distributions $\mathscr{P} = \{ \mathcal{P}_x\}_{x\in\Omega}$.  These distributions define a notion of ``closeness" that is relevant to the application at hand. While it is hard to reason about all possible perturbation ensembles that arise in practice, we believe that for all ``reasonable" ensembles, $\mathscr{A}$ performs well in the following quantitative sense: 

%We formally state our conjecture for \textsc{ComputeAnchor}.

\begin{conjecture}[$\mathscr{A}$ performs well for all reasonable perturbation ensembles]
    \label{conj: anchors}
     Let $f:\Omega \to \bits$ be a blackbox model, $\mathcal{D}$ be a distribution over $\Omega$,  and $\eps,\delta \in (0,1)$. Let $\mathscr{P} = \{ \mathcal{P}_x\}_{x\in\Omega}$ be a ``reasonable" ensemble of perturbation distributions.  With probability at least $1 - \delta$ over the choice of $\bx\sim\mathcal{D}$, the anchor-finding algorithm $\mathscr{A}$ returns an $O(\eps)$-error anchor for $\bx$ of size $\poly(\mathcal{A}(f,\eps),1/\eps,1/\delta)$.
\end{conjecture}


We note the dimension-independent bound on the size of the anchors.  As discussed in~\Cref{sec:compare},~\cite{RSG18}'s algorithm is such that even under favorable distributional and feature assumptions, there are functions $f$ for which $\mathcal{A}(f) = 2$ and yet their algorithm returns anchors of size $\Omega(d)$. 

As progress towards understanding~\Cref{conj: anchors}, we focus on a natural and generic perturbation ensemble (the ``independent perturbation ensemble",~\Cref{def:independent perturbation ensemble}) which we believe serves as a good proxy for many perturbation ensembles of interest.  We prove a special case of~\Cref{conj: anchors} for this ensemble under distributional and feature assumptions.  

%In the remainder of this section, we prove \Cref{conj:implicit dt} and \Cref{conj: anchors} when $\Omega = \bits^d$ and $\mathcal{D}$ is the uniform distribution over $\bits^d$.

%In this section we give provable guarantees for the runtime and query complexity of {\sc ComputeAnchor} when $\Omega_i = \{\pm 1\}$ and $\mathcal{D}$ is the uniform distribution, $\{\pm 1\}^d$. 

% \textbf{Do we want this here?}
% \begin{theorem}
% \label{thm:main}
% {\sc ComputeAnchor} has the following guarantee. Let $f : \bits^d \to \bits$ be a blackbox model.  Given an instance $\underline{x} \in \bits^d$, parameters $\eps,\gamma \in (0,1)$, and query access to $f$, {\sc ComputeAnchor} makes $\poly(A(f),1/\eps,1/\gamma)$ many queries to $f$ and either 
% \begin{itemize}
% \item[$\circ$] outputs a $(1-\gamma)$-precise $f$-anchor for $\underline{x}$, or 
% \item[$\circ$] fails and outputs ``$\bot$".  
% \end{itemize} The fraction of instances $x$ on which {\sc ComputeAnchor} outputs $\bot$ is at most $\eps$. 
% \end{theorem}



% \subsection{Certificate and decision tree complexities, and Smyth's theorem} 
% \lnote{Move this up to before Section 3}

% \violet{Our notion of certificates as defined in~\Cref{def:anchors} is {\sl local}, specific to each instance $x$, whereas Smyth's theorem concerns a {\sl global} notion of certificates, defined for the entire function $f$.  %In this section we state Smyth's theorem and relate these two notions of certificates. 
% }

% \violet{ 
% \paragraph{Notation.} Fix a function $f : \bits^d\to\bits$ and let $\mathscr{C}$ be a collection of subsets $C\sse [d]$.  We write `$x\models \mathscr{C}$' if there exists $C\in\mathscr{C}$ such that $C$ is a $0$-error certificate for $x$: 
% \[ f(y) = f(x) \text{ for all $y\in\bits^d$ such that $y_C = x_C$},\]
% and we write `$x\not\models\mathscr{C}$' otherwise. 
% }

% \violet{
% Given two collections $\mathscr{C}_1$ and $\mathscr{C}_{-1}$ of subsets, we define a corresponding function $\Phi_{\mathscr{C}_1,\mathscr{C}_{-1}} : \bits^d \to \{\pm 1,\bot\}$ as follows: 
% \[ 
% \Phi_{\mathcal{C}_1,\mathcal{C}_{-1}}(x) = 
% \begin{cases} 
% 1 & \text{if $x \models \mathscr{C}_1$ and $x\not\models\mathscr{C}_{-1}$} \\
% -1 & \text{if $x \models \mathscr{C}_{-1}$ and $x\not\models\mathscr{C}_1$} \\
% \bot & \text{otherwise.}
% \end{cases} 
% \] 
% \begin{definition}[Certificate complexity] 
% The {\sl global $\eps$-error certificate complexity} of $f : \bits^d\to\bits$, denoted $\mathcal{C}_\eps(f)$, is the smallest $k$ for which there exists two collections $\mathscr{C}_1$ and $\mathscr{C}_{-1}$ of size-$k$ subsets satisfying $\Pr[f(\bx)\ne \Phi_{\mathscr{C}_1,\mathscr{C}_{-1}}(\bx)] \le \eps$. 
% \end{definition} 


%  \begin{definition}[Decision tree complexity]
%      \label{def:optimal dt depth}
%      The {\sl $\eps$-error decision tree complexity} of $f: \bits^d \to \bits$, denoted $D_\eps(f)$, is the smallest $k$ for which there exists a depth-$k$ decision tree $T$ satisfying $\Pr[T(\bx) \neq f(\bx)] \leq \eps$.
%  \end{definition}
 
%  It is straightforward to verify that $C_\eps(f) \le D_\eps(f)$ for all $f : \bits^d \to \bits$ and $\eps > 0$.  
 
 
%  Smyth, resolving a longstanding conjecture of Tardos~\cite{Tar89}, gives a surprising converse to this inequality: 


% \begin{theorem}[\cite{Smy02}]
% For all $f: \bits^d\to\bits$ and $\eps > 0$ we have that \[ D_\eps(f) \le O(C_{\eps^3/30}(f)^2/\eps^3). \] 
% \end{theorem}

% }


% \gray{ 
% A key ingredient in our proof is a result of Symth \cite{Smy02} from complexity theory.  Smyth's theorem concerns {\sl certificate complexity},   which can be viewed as a ``global" variant of anchor complexity.  

% \begin{definition}[Certificates] A {\sl certificate} of a $d$-dimensional instance space $\Omega = \Omega_1\times \cdots \times \Omega_d$ is a function $c$ with domain $A \sse [d]$ such that $c(i) \in \Omega_i$ for all $i \in A$.  The {\sl size} of the certificate is $|A|$, and we say that an instance $x\in \Omega$ {\sl satisfies $c$}, denoted $x \models c$, if $x_i = c(i)$ for all $i\in A$.  
% \end{definition} 
% {\bf Notation.}  For a set $\mathcal{C}$ of certificates, we write $x\in \mathcal{C}$ if there exists $c\in \mathcal{C}$ such that $x \models c$, and we write $x\notin \mathcal{C}$ otherwise.  For two sets of certificates $\mathcal{C}_1$ and $\mathcal{C}_{-1}$ over $\Omega$, we define a corresponding function $\Phi_{\mathcal{C}_1,\mathcal{C}_{-1}} : \Omega \to \{\pm 1,\bot\}$ as follows: 
% \[ 
% \Phi_{\mathcal{C}_1,\mathcal{C}_{-1}}(x) = 
% \begin{cases} 
% 1 & \text{if $x \in \mathcal{C}_1$ and $x\notin\mathcal{C}_{-1}$} \\
% -1 & \text{if $x \in \mathcal{C}_{-1}$ and $x\notin\mathcal{C}_1$} \\
% \bot & \text{otherwise.}
% \end{cases} 
% \] 


% \begin{definition}[Certificate complexity]
% Let $f : \Omega\to\bits$ be a function and $\mathcal{D}$ be a distribution over $\Omega$.  The {\sl $\eps$-error certificate complexity of $f$}, denoted $C_\eps(f)$, is the smallest $k$ such that there exists two collections of size-$k$ certificates $\mathcal{C}_1$ and $\mathcal{C}_2$ satisfying $\Prx_{\bx\sim\mathcal{D}}[f(\bx)\ne \Phi_{\mathcal{C}_1,\mathcal{C}_{-1}}(\bx)] \le \eps.$ 
% \end{definition} 
% % \begin{definition}[Global anchor complexity] 
% % Let $f : \Omega \to \bits$ be a function and  $\mathcal{D}$ be a distribution over $\Omega$.  We say that $f$ has {\sl global $\eps$-error anchor complexity $k$} if the following holds. 

% % Let $\mathcal{S}_1$ and $\mathcal{S}_{-1}$ be two collections of size-$k$ anchors. Define a corresponding function $g : \Omega\to\{-1,1,\bot\}$ as follows: 

% % \end{definition} 

% % %A theorem of \cite{Smy02} allows us to bound the size of anchors produced by our algorithm. This theorem bounds the optimal decision tree size of a function in terms of its \emph{global anchor complexity}. We define global anchor complexity and state Smyth's theorem below: 

% % \begin{definition}[Global anchor complexity]
% % Let $f:\Omega \to \bits$ be any function. A set of anchors $A^{\star}(f)$ is a size-$k$, $\eps$-error global anchor set if each anchor $A_x \in A^{\star}$ has size at most $k$ and
% % \[\Pr_{\bx \sim \mathcal{D}} [(\bx, f) \text{ has a 0-error anchor }A_x \in A^{\star}(f)] \ge 1 - \eps\]

%  \begin{definition}[Decision tree complexity]
%      \label{def:optimal dt depth}
%      Let $f: \Omega \to \bits$ and $\mathcal{D}$ be a distribution over $\Omega$. The {\sl $\eps$-error decision tree depth}, denoted $D_\eps(f)$, is the smallest $k$ for which there exists a depth-$k$ decision tree $T$ satisfying $\Prx_{\bx \sim \mathcal{D}}[T(\bx) \neq f(\bx)] \leq \eps$.
%  \end{definition}


% We are now ready to state Smyth's theorem, which relates the certificate and decision tree complexities of a function:  


% \begin{theorem}[\cite{Smy02}]
% Let $f: \Omega\to\bits$ be a function and $\mathcal{D}$ be a product distribution over $\Omega$. For all $\eps \in (0,1)$ we have that $D_\eps(f) \le O(C_{\eps^3/30}(f)^2/\eps^3)$.
% \end{theorem} 

% % \begin{theorem}[\cite{Smy02}]
% % \label{thm:smyth}
% % Let $\eps > 0$ and let $f: \Omega^d \to \{\pm1\}$ be a function with $\eps$-error global anchor complexity $\mathcal{A}^\star(f, \eps)$. Then there exists a decision tree $T$ such that $T$ is $\eps$-close to $f$ and $\mathrm{depth}(T) \le K \cdot (\mathcal{A}^\star(f, \eps)^2)$, for constant $K$.
% % \end{theorem}
 
 
% We derive as a corollary of Smyth's theorem a relationship between anchor and decision tree complexities: 

% \begin{corollary}[Bounding decision tree complexity in terms of anchor complexity]
% \label{cor:smyth corollary}
% Let $f : \Omega\to\bits$ be a function and $\mathcal{D}$ be a product distribution over $\Omega$.  For any $\eps \in (0,1)$, we have $D_{\eps}(f) \le O(\mathcal{A}(f)^2/\eps^9)$.
% \end{corollary} 

% \begin{proof} 
% Let $k \coloneqq \mathcal{A}(f)$.  By Markov's inequality, we have that $\Pr_{\bx\sim\mathcal{D}}[\mathcal{A}(f,\bx)\le 30k/\eps^3] \ge 1-(\eps^3/30)$.  For every $x\in f^{-1}(1)$ (resp.~$x\in f^{-1}(-1)$) that contributes to this probability, we include in $\mathcal{C}_1$ (resp.~$\mathcal{C}_{-1}$) the certificate corresponding to $x$'s anchor of size $30k/\eps^3$.  It follows that $\Prx_{\bx\sim\mathcal{D}}[f(\bx)\ne \Phi_{\mathcal{C}_1,\mathcal{C}_{-1}}(\bx)] \le \eps^3/30$ and hence $C_{\eps^3/30}(f) \le 30k/\eps^3$.  By Smyth's theorem,  
% \[ D_{\eps}(f) \le O(C_{\eps^3/30}(f)^2/\eps^3) = O(k^2/\eps^9) \] 
% and this completes the proof. 
% \end{proof} 

% }

% \begin{lemma} 
% Let $f: \Omega^d \to \{\pm1\}$ be a function with 0-error anchor complexity $\mathcal{A}(f,0)$. Then for any $\eps > 0$, there exists a decision tree $T$ such that $T$ is $\eps$-close to $f$ and $\mathrm{depth}(T) \le K\cdot (\mathcal{A}(f,0)/\eps)^2$, for constant $K$.
% \end{lemma}

% \begin{proof}
% Recall that $\mathcal{A}(f) = \E_{\bx \sim \mathcal{D}} [\mathcal{A}(f, \bx)]$. By Markov's inequality, we have $\Pr_{\bx \sim \mathcal{D}} [\mathcal{A}(f, \bx) \le \mathcal{A}(f, 0)/\eps] \ge 1 - \eps$. For each $x$ such that $\mathcal{A}(f,x,0) \le \mathcal{A}(f,0)/\eps$, let $A_x$ be the smallest 0-error anchor for $x$. Let $A^{\star}(f)$ be the set of anchors $\{A_x~|~\{\mathcal{A}(f,x,0) > \mathcal{A}(f,0)/\eps\}$. Then $A^{\star}(f)$ is a size-$\mathcal{A}(f,0)/\eps$, $\eps$-error global anchor for $f$, and thus: 
% \[\mathcal{A}^{\star}(f, \eps) \le \mathcal{A}(f,0)/\eps\].
% Applying \Cref{thm:smyth} yields a decision tree of depth $O((\mathcal{A}(f,0)/\eps)^2)$ that $\eps$-approximates $f$.
% \end{proof}

\gray{
\subsection{The independent perturbation distribution and proving a special case of~\Cref{conj: anchors}}

\begin{definition} 
[The independent perturbation ensemble]
    \label{def:independent perturbation ensemble}
    Let $\mathcal{D}$ be a distribution over an instance space $\Omega$.  Let $p\in (0,1)$ be a noise rate, and $\mathscr{P}^{(p)}_{\mathrm{ind}} = \{ \mathcal{P}_x\}_{x\in\Omega}$ be the ensemble where for each $x\in \Omega$, a draw $\bx'\sim \mathcal{P}_x$ is formed by independently rerandomizing each feature of $x$ with probability $p$ according to the marginal of $\mathcal{D}$ on that feature.
\end{definition} 

% \begin{definition}[The independent perturbation distribution ensemble]
%     \label{def:independent perturbation ensemble}
%     Fix some noise rate $p$, and for any $x \in \bits^d$ let $\mathcal{P}^{(p)}_x$ be the distribution which takes a copy of $x$ and for each coordinate, with probability $p$, independently rerandomizes it. This means, for $x' \sim \mathcal{P}^{(p)}_x$, each coordinate of $x'$ is independent and $x'_i = x$ with probability $1 - \frac{p}{2}$. We define the independent perturbation distribution ensemble at noise rate $p$, denoted $\mathscr{P}_{\mathrm{ind}}^{(p)}$ to be the ensemble $\{\mathcal{P}^{(p)}_x\}_{x \in \bits^d}$.
% \end{definition}

In the remainder of this section, we work in the setting of binary features ($\Omega = \bits^d$) and with $\mathcal{D}$ being the uniform distribution. 
We leverage a recent structural result that bounds the distance between $f$ and the greedy noise stabilizing decision tree $\Upsilon_f^{k,\eta}$ (\Cref{def:approximate noise stabilizing tree}) when the latter is defined with respect to $\mathscr{P}^{(p)}_{\mathrm{ind}}$. 

%\subsection{The~\cite{BLT-test} structural result} 

%\subsection{Proof of \Cref{thm:main}}
\begin{lemma}[Lemma 2.6 of \cite{BLT-test}]%\footnote{\cite{BLT-test} write their result in terms of the size of a tree that is close to $f$, rather than the depth. Here, we translate their results to depth. It's easy to see from their proof that everything follows with depth instead of size (indeed some steps simplify). Furthermore, their result has $\eps^2$ in the denominator instead of $\eps^3$, but through personal communication with the authors, we know that they plan to update their proof, fixing a minor bug, which will lead to an $\eps^3$ as we write.}]
%\label{lem:DT structural results}
Let function $f: \bits^d \to \bits$ be a function.  Consider  $\Upsilon_f^{k,\eta}$ where $k=O((D_\eps(f)/\eps)^3)$ and $\eta = \Theta(1/k)$, defined with respect to $\mathscr{P}^{(p)}_{\mathrm{ind}}$ at noise rate $p = O(\eps/D_\eps(f))$. Then $\Pr[\Upsilon_f^{k,\eta}(\bx) \ne f(\bx)] \le O(\eps)$.
\end{lemma}


With~\Cref{lem:DT structural results} in hand we now put the pieces together and establish the following special case of~\Cref{conj: anchors}: 

\begin{theorem} 
Let $f : \bits^d\to\bits$ be a function and $\eps,\delta\in (0,1)$.  With probability at least $1-\delta$ over $\bx\sim\bits^d$, our anchor-finding algorithm $\mathscr{A}$ returns an $\eps$-error anchor of size $\poly(\mathcal{A}(f),1/\eps,1/\delta)$.    
\end{theorem} 

\begin{proof} 
Applying Smyth's theorem,~\Cref{cor:smyth corollary}, we have the bound 
\[ D_{\eps\delta}(f) \le O(\mathcal{A}(f)^2/(\eps\delta)^9).  \]
Combining this with~\cite{BGLT-NeurIPS1}'s structural theorem,~\Cref{lem:DT structural results}, we get that
\begin{enumerate} 
\item $\Pr[\Upsilon^{k,\eta}_f(\bx)\ne f(\bx)] \le O(\eps\delta)$, where 
\item $k \le O((D_{\eps\delta}(f)/\eps)^3) \le \poly(\mathcal{A}(f),1/\eps,1/\delta).$
\end{enumerate} 
These correspond exactly to the two items in the assumption of~\Cref{lem:learning-to-anchor-finding} with `$T$' being $\Upsilon^{k,\eta}_f$, and the theorem follows.
\end{proof} 
}


% Given the above structural result, we are easily able to prove a special case of \Cref{conj:implicit dt}.
% \begin{theorem}[Special case of \Cref{conj:implicit dt}]
%     \label{thm:decision tree special case}
%     Given any black box model $f: \bits^d \to \bits$ and desired accuracy $\eps > 0$. For $p = \frac{\eps}{\depth_\eps(f)}$ and $k = \left(\frac{\depth_\eps(f)}{\eps}\right)^3$, if we use $\mathscr{P}_{\mathrm{ind}}^{(p)}$ as our perturbation distribution and the algorithm in \Cref{lem:our-implicit-alg} to learn an implicit decision tree $T$, then $\Pr_{\bx \sim \bits^d}[T(\bx) \neq f(\bx)] \leq \eps$. 
% \end{theorem}
% \begin{proof}
%     In \Cref{lem:our-implicit-alg}, we proved that our algorithm will be the decision tree $\Upsilon_f^{k, 1/k}$. By \Cref{lem:DT structural results}, this tree is $O(\eps)$-close to $f$.
% \end{proof}


% Next, we prove a special case of \Cref{conj: anchors}. This proof leverages Smyth's theorem (\Cref{lem:smyth corrolary}), \Cref{thm:decision tree special case}, and \Cref{lem:learning-to-anchor-finding}.
% \begin{theorem}[Special case of \Cref{conj: anchors}]
%     Let $f: \bits^d \to \bits$ be a function, $\eps > 0$ a desired precision, and $\delta > 0$ a failure probability. Given random input $\bx \sim \bits^d$, using the algorithm in \Cref{lem:our-implicit-alg} to learn an implicit decision tree for $f$ and then \textsc{ComputeAnchor} from \Cref{lem:learning-to-anchor-finding}, for appropriately chosen parameters, returns an $\eps$-error anchor of size at most $k = \frac{\mathcal{A}(f)^6}{\eps^9}$ with probability at least $1 - \delta$ over the choice of $\bx$.
%     %Let  be the algorithm that, on input $x$, uses \Cref{lem:our-implicit-alg} with perturbation distribution $\mathscr{P}_{\mathrm{ind}}^{(p)}$ and $p = \frac{\mathcal{A}(f)^2}{\eps^3}$ to create an implicit decision tree, $T$, of depth $k = \textbf{todo}$ and then outputs the result of $\textsc{FindAnchor}(f, T, x, \eps, \delta)$. If $\bx$ is chosen randomly from $\bits^d$, then with probability at least $1 - \delta$, $\mathcal{A}(\bx)$ returns an $\eps$-error anchor of size at most $d$.
% \end{theorem}
% We specify the parameters for \Cref{lem:learning-to-anchor-finding} and \textsc{ComputeAnchor} in the below proof.
% \begin{proof}
%     By Smyth's theorem, we have $\depth_\eps(f) \le K\cdot (\mathcal{A}(f)/\eps)^2$ for some constant $K$. Then by \Cref{thm:decision tree special case}, the algorithm in \Cref{lem:our-implicit-alg} learns an implicit decision tree $T$ such that 
%     \begin{align*}
%         \Pr_{\bx \sim \bits^d}[T(\bx) \neq f(\bx)] \leq \eps.
%     \end{align*}
%     and 
%     \begin{align*}
%         \depth(T) \le \left(\frac{\depth_\eps(f)}{\eps}\right)^3 \le \frac{\mathcal{A}(f)^6}{\eps^9}
%     \end{align*}
%     Then by \Cref{lem:learning-to-anchor-finding}, \textsc{ComputeAnchor} finds an $\eps$-error anchor of size at most $\frac{\mathcal{A}(f)^6}{\eps^9}$, with probability at least $1 - \delta$.
% \end{proof}

==> intro.tex <==
%!TEX root = explainability.tex

\begin{abstract}
We consider the problem of explaining the predictions of an arbitrary blackbox model $f$.  Given query access to $f$ and an instance $x$, the goal is to output an explanation of {\sl why} $f$ assigns $x$ the label $f(x)$: a set of $x$'s features that in conjunction essentially determines~$f(x)$. Such explanations were introduced in the recent work of Ribero, Singh, and Guestrin~\cite{RSG18} who demonstrated, through experiments and user studies, their effectiveness across diverse domains and applications. 

%We introduce a framework to rigorously analyze and compare the quality of algorithms for this task.  Within this framework, 

%\violet{We bridge a connection between the problem of efficiently finding such explanations and that of {\sl implicitly learning decision trees}, a new algorithmic problem that we introduce.  Decision trees are the canonical example of an interpretable  model, and the implicit nature of this task allows for efficient algorithms even when the complexity of~$f$ necessitates an intractably large surrogate decision tree. We then solve the implicit learning problem by bringing together techniques from learning theory, local computation algorithms, and complexity theory, and leveraging recent advances in the design of decision tree learning algorithms with provable guarantees.  We thereby obtain an efficient explanation-finding algorithm with provable guarantees on the succinctness and precision of the explanations that it returns.}
%



We design an efficient algorithm for computing such explanations with provable guarantees on the succinctness and precision of the explanations that it returns.
We do so by bridging a connection to the problem of {\sl implicitly learning decision trees}, a new algorithmic problem that we introduce.  Decision trees are the canonical example of an interpretable  model, and the implicit nature of the learning task allows for efficient algorithms even when the complexity of~$f$ necessitates an intractably large surrogate decision tree. We then solve the implicit learning problem by bringing together techniques from learning theory, local computation algorithms, and complexity theory, and by leveraging recent advances in the design of decision tree learning algorithms with provable performance guarantees.

%We design an efficient algorithm for finding succinct and precise explanations.  We do so by bridging a connection between the problem of explaining blackboxes and that of {\sl implicitly learning decision trees}, a new algorithmic problem that we introduce.  Decision trees are the canonical example of an interpretable  model, and the implicit nature of this task allows for efficient algorithms even when the complexity of~$f$ necessitates an intractably large surrogate decision tree.  We then solve the implicit learning problem by bringing together techniques from learning theory, local computation algorithms, and complexity theory. 

Our overall approach of ``explaining by implicit learning" shares elements of two previously disparate methods for post-hoc explanations, {\sl global} and {\sl local} explanations, and we make the case that it enjoys advantages of both.  
\end{abstract}

% \thispagestyle{empty}

% \newpage
% \setcounter{page}{1}



\section{Introduction} 


Modern machine learning systems have access to staggering amounts of computational resources and data, enabling them to rapidly train increasingly sophisticated and complex models. These models achieve remarkable performance on a wide range of tasks, but their success appears to come at a  price: the complexity of these models,  responsible for their expressivity and accuracy, makes their inner workings inscrutable to human beings, rendering them powerful but opaque blackboxes.  As these blackboxes become increasingly central in mission-critical systems and their predictions increasingly relied upon in high-stakes decisions, there is a growing urgency to address their lack of interpretability~\cite{DK17,Lip18}.  


There has therefore been a  surge of interest in the problem of {\sl explaining} the predictions of blackbox models: {\sl why} did a model $f$ assign an instance $x$ the label $f(x)$?   While there are numerous possibilities for what qualifies as an explanation~\cite{SK10,BSHKHM10,SVZ14,RSG16,KL17,LL17,STY17,RSG18}, in this work we consider an explanation to be a set of $x$'s features that in conjunction essentially determines~$f(x)$.  Recent work of Ribeiro, Singh, and Guestrin~\cite{RSG18} introduced such explanations and termed them {\sl anchors}, and advocated for them for their ease of understanding by human beings and clarity of scope.~\cite{RSG18} showed, through experiments and user studies, the effectiveness of anchors across a variety of domains and tasks, and also highlighted several advantages of anchors over LIME explanations~\cite{RSG16}.
%As a motivating example, consider a classifier $f$ for a loan approval decision, mapping individuals to a binary decision (approval or denial), and suppose~$f$ denies an individual~$x$ the loan.  We consider an explanation for this decision to be a set $A$ of $x$'s features---say their income, credit score, and history of default---that in conjunction is  responsible for $f$'s decision to deny $x$ the loan.  

We seek {\sl succinct} and {\sl precise} anchors. Intuitively, this means that we would like  the set of features to be as small as possible, and for it to nonetheless be a sufficient explanation for $f(x)$ with high probability; more formally, we have the following definition: 

\begin{definition}[Succinct and precise anchors] 
\label{def:anchors} 
Let $f : \Omega \to \bits$ be a classifier over a $d$-dimensional instance space, $\mathcal{D}$ be a distribution over $\Omega$, and $x \in \Omega$ be an instance. We say that a set $A\sse [d]$ of features is a {\sl size-$k$ $\eps$-error anchor for $x$} if both of the following hold: 
\begin{itemize} 
\item[$\circ$] {\sl Succinctness:} $|A| \le k$, 
\item[$\circ$] {\sl Precision:} $\ds \Prx_{\by\sim \mathcal{D}}\big[f(\by) \ne f(x)\mid \by_A = x_A\big] \le \eps$.
\end{itemize} 
 \end{definition} 

%(There are subtle differences between our definition and the one in~\cite{RSG18}; see [...] for a comparison and discussion.)  

Succinctness and precision are both desirable properties of explanations, but they are inherently in tension with each other.  For any instance $x$, the complete anchor $A = [d]$ has perfect precision ($\eps = 0$) but is not succinct; on the other hand, the empty anchor $A = \emptyset$ is certainly succinct ($k = 0$) but has poor precision.  The challenge is therefore to understand and balance this tension, and to design algorithms that simultaneously optimize for both desiderata.   We are now ready to state the algorithmic problem that we consider in this work: 
\begin{quote} 
{\sl Given query access to a blackbox model $f$ and an instance $x$, efficiently find a succinct and precise anchor for $x$.}
\end{quote}

We focus on algorithms that are {\sl model agnostic}, requiring no assumptions about the structure of $f$.  This stands in contrast to algorithms that are tailored to explaining specific classes of models (e.g.~neural networks or random forests).  %The algorithms that we design and analyze can therefore be employed to explain the predictions of any classifier. 




\subsection{Our contributions}
\label{sec:our-contributions} 
The experimental results of~\cite{RSG18}, supporting the effectiveness of anchors across domains and applications, motivate the development of efficient anchor-finding algorithms with provable guarantees on the succinctness and precision of the anchors that they return.  We design such an algorithm in this work.  We do so by first bridging a connection between the problem of finding anchors and that of {\sl implicitly learning decision trees}, a new algorithmic problem that we introduce.  We then solve the implicit learning problem by bringing together techniques from learning theory, local computation algorithms, and complexity theory, and by leveraging recent advances in the design of decision tree learning algorithms with provable performance guarantees.  In more detail, our contributions are as follows: 

\begin{itemize}[leftmargin=15pt] 
    \item[$\circ$] {\sl The problem of implicitly learning decision trees.}  Decision trees are the canonical example of an interpretable model.  Their predictions admit simple explanations:  an anchor for an instance~$x$ is the root-to-leaf path in the tree that $x$ follows.   A natural and well-studied approach to explaining a blackbox model~$f$ is therefore to first learn a decision tree $T$ that well-approximates~$f$, and with this surrogate decision tree $T$ in hand, one can then output an anchor for any instance $x$ by returning the corresponding path in~$T$~\cite{CS95,BS96,AB07,ZH16,VLJODV17,BKB17,VS20}. 
  A limitation of this approach lies in fact that many models of interest are inherently complex and cannot be well-approximated by a decision tree of tractable size. % (e.g.~models for text or image applications almost certainly do not admit such approximations). 



Towards circumventing this limitation, we introduce the problem of {\sl implicitly} learning  decision trees.  Roughly speaking, an algorithm for this task allows one to efficiently navigate a surrogate decision tree $T$ for $f$---{\sl without building $T$ in full}.  With such an algorithm, the complexity of finding an anchor scales with the {\sl depth} of $T$, making it exponentially more efficient than building $T$ in full, the complexity of which scales with its  overall {\sl size}.  



    \item[$\circ$]  {\sl Efficient algorithms.}   We design an efficient algorithm for implicitly learning decision trees, and from it we derive an algorithm for finding anchors.  The latter algorithm constructs an anchor $A$ for an instance $x$ by adding to $A$ the most ``important" feature of~$f$ and recursing on the subfunction determined by $x$'s value for that feature.  Our notion of feature importance generalizes a {\sl noise stability} based definition introduced by Blanc, Gupta, Lange, and Tan in the context of (non-implicit) decision tree learning~\cite{BGLT-NeurIPS1}.  Our resulting algorithm is similar in spirit to a greedy anchor-finding algorithm proposed in~\cite{RSG18}, with a number of key differences which we show are crucial for the performance guarantees that we establish.      

     \item[$\circ$] {\sl Provable performance guarantees.}    We analyze the performance our algorithms under distributional and feature assumptions. We first prove a quantitatively optimal relationship between the ``anchor complexity" of a function $f$ and the depth of the best decision tree that approximates it.  We derive this as a corollary of a deep result from complexity theory, Smyth's theorem~\cite{Smy02}; a key observation here is a close correspondence between anchors and the notion of {\sl certificates} in complexity theory.  We combine this with a new structural lemma about decision trees, established by Blanc, Lange, and Tan in the context of local computation algorithms~\cite{BLT-test}, to derive performance guarantees for our implicit learning algorithm.  This in turn yields guarantees on the succinctness and precision of the anchors that our anchor-finding algorithm returns. 
    
    \end{itemize} 


%     For a given accuracy parameter $\eps$, we define the {\sl expected $\eps$-error anchor complexity of $f$} to be the expected size of the smallest $\eps$-error anchor for a random instance $\bx \sim \mathcal{D}$.  This will serve as our benchmark: we would like the size of the anchor that our algorithm returns to be as close to this quantity as possible.  With this goal and the bullet above in mind,  we are faced with two questions: 1) If $f$ has expected anchor complexity $k$, can it be well-approximated by a decision tree whose depth is bounded by a function of $k$?  2) If so, can we give an efficient algorithm for implicitly learning this decision tree? 
%     
%    \begin{itemize}[leftmargin=15pt]
%    
%    \item[$\circ$] {\sl Anchor complexity and decision tree complexity.}  We give a quantitatively optimal answer to the first question in the case of product distributions, deriving our bound as a corollary of a deep result from complexity theory, Symth's theorem~\cite{Smy11}.  [...] equivalence between 
%    
%    \item[$\circ$]  {\sl Efficient algorithms.}   We give an efficient algorithm for implicitly learning decision trees, and from it we derive an algorithm for finding anchors.  Our algorithm constructs an anchor $A$ for an instance $x$ by adding to $A$ the most ``important" feature of~$f$ and recursing on the subfunction determined by $x$'s value for that feature.  We use a {\sl noise stability} based notion of feature importance introduced by Blanc, Gupta, Lange, and Tan in the context of (non-implicit) decision tree learning~\cite{BGLT-NeurIPS1}.  Our algorithm is similar in spirit to a greedy algorithm proposed in~\cite{RSG18} with a number of key differences.  We show that these differences are crucial for the performance guarantees that we establish.      
%
%     \item[$\circ$] {\sl Provable performance guarantees.}    We analyze our algorithm under the assumption of binary features and product distributions, and derive strong guarantees on the succinctness and precision of the anchors that it returns.  Our proof draws on techniques from complexity theory and property testing.  We first show a sharp relationship between the expected anchor complexity of $f$ and the depth of the best decision tree that approximates it; we derive this as a corollary of a deep result in complexity theory, Symth's theorem~\cite{Smy11}.  We combine this with a new structural fact about decision trees, established by Blanc, Lange, and Tan in the context of property testing~\cite{BLT-test}. %In addition to its time efficiency, our algorithm is also highly query efficient, with the number of queries to $f$ scaling {\sl polylogarithmically} with the dimension of the instance space and the size of the surrogate decision tree. 
%   
%    
%    
%%\item[$\circ$] {\sl Anchor complexity and decision tree complexity.}  For a given accuracy parameter $\eps$, we define the {\sl expected $\eps$-error anchor complexity of $f$} to be the expected size of the smallest $\eps$-error anchor for a random instance $\bx \sim \mathcal{D}$.  This will be the benchmark for the quality of our algorithm: we would like the size of the anchor that our algorithm returns to be as close to this quantity as possible. 
%%
%%With this goal and the previous bullet in mind, we are faced with the following question: what is the relationship between the expected anchor complexity of $f$ and its approximate decision tree complexity, the depth of the shallowest decision tree that approximates $f$?  In the case of product distributions, we give a sharp answer to this question by drawing on a deep result from complexity theory, Symth's theorem~\cite{Smy11}.
%
%    
%    \item[$\circ$] {\sl Provable performance guarantees.}    We establish strong performance guarantees for our algorithm in the case of binary features and product distributions: for all error parameters $\eps$ and instances $x$, our algorithm always returns an $\eps$-error anchor for $x$, and furthermore, the expected size of the anchor that our algorithm returns is polynomially bounded by the expected $O(\eps)$-error anchor complexity of $f$.   Our proof draws on techniques from complexity theory and property testing.  We first show a sharp relationship between the expected anchor complexity of $f$ and the depth of the best decision tree that approximates it; we derive this as a corollary of a deep result in complexity theory, Symth's theorem~\cite{Smy11}.  We then combine this with a new structural fact about decision trees, established by Blanc, Lange, and Tan in the context of property testing~\cite{BLT-test}, to bound the size of the anchors that our algorithm returns.  %In addition to its time efficiency, our algorithm is also highly query efficient, with the number of queries to $f$ scaling {\sl polylogarithmically} with the dimension of the instance space and the size of the surrogate decision tree. 

    
%\end{itemize}


\subsection{Prior work and discussion: global versus local explanations}  
\label{sec: global vs local explanations}
Existing approaches to post-hoc explanations mostly fall into two categories.  {\sl Global explanations} seek to capture the behavior of the entire model $f$, often by approximating it with a simple and interpretable model such as a decision tree~\cite{CS95,BS96,AB07,ZH16,VLJODV17,BKB17,VS20} or a set of rules~\cite{LKCL19,LAB20}.  A limitation of such approaches, alluded to above and also discussed in numerous prior works (see e.g.~\cite{RSG16,RSG18}),  is that complex models often cannot be well-approximated by simple ones.  In other words, using a simple surrogate model necessarily results in low fidelity to the original model.  


Our work falls in the second category of {\sl local explanations}~\cite{SK10,BSHKHM10,SVZ14,RSG16,KL17,LL17,RSG18}.  These seek to explain $f$'s label for specific instances $x$.  Several of these approaches are based on notions of $f$ being ``simple around $x$": for example, LIME explanations~\cite{RSG16} show that $f$ is ``approximately linear around $x$", and anchors, introduced in~\cite{RSG18} and the focus of our work, show that $f$ is ``approximately constant in a subspace containing $x$".  The corresponding algorithms can therefore be run on models that are too complex to be faithfully represented by a simple global surrogate model. 


While our work falls in the category of local explanations, we believe that our new approach of ``explaining by implicit learning" enjoys advantages of both local and global methods.  The local explanations that our algorithm returns are all  consistent with a {\sl single} decision tree $T$ that well-approximates $f$ globally.  The implicit nature of the learning task allows for $T$ to be intractably large, hence allowing for corresponding algorithms to be run on complex models $f$, circumventing the limitation of global methods discussed above.   On the other hand, the existence of a single global surrogate decision tree, albeit one that may be too large to construct in full, affords several advantages of global methods.  We list a few examples: 
\begin{itemize}[leftmargin=15pt] 
\item[$\circ$]  {\sl Partial information about global structure.} Our implicit learning algorithm can efficiently construct the subgraph of $T$ comprising the root-to-leaf paths of a few specific instances; alternatively, it can construct the subtree of $T$ rooted at a certain node, or the first few layers of~$T$.  All of these could shed light on the global behavior of~$f$.
\item[$\circ$]  {\sl Feature importance information.}  Our implicit decision tree $T$ has useful properties beyond being a good approximator of $f$.  As we will show, its structure carries valuable semantic information about $f$, since the feature queried at any internal node $v$ is the most ``noise stabilizing" feature of the subfunction $f_v$.   The features in the anchors that our algorithm returns can be ordered accordingly, each being the most noise stabilizing feature of the subfunction determined by $x$'s value on the previous features.  
\item[$\circ$] {\sl Measures of similarity between instances.}  Every decision tree $T$ naturally induces a ``similarity distance" between instances, given by the depth of their lowest common ancestor within $T$.  Therefore pairs of instances that share a long common path in $T$ before diverging (or do not diverge at all) are considered very similar, whereas pairs of instances that diverge early on, say at the root, are considered very dissimilar. (Such tree-based distance functions have been influential in the study of hierarchical clustering; see e.g.~\cite{Das16}.)  This distance between two instances can be easily calculated from the anchors that our algorithm returns for them. 

\end{itemize} 



\subsection{Preliminaries} 

For two functions $f,g : \Omega \to \bits$ and a distribution $\mathcal{D}$ over $\Omega$, we say that $f$ and $g$ are {\sl $\eps$-close with respect to $\mathcal{D}$} if $\Pr_{\bx\sim\mathcal{D}}[f(\bx)\ne g(\bx)] \le \eps$. 


